New efficient algorithms for multiple change-point detection with kernels

Several statistical approaches based on reproducing kernels have been proposed to detect abrupt changes arising in the full distribution of the observations and not only in the mean or variance. Some of these approaches enjoy good statistical properties (oracle inequality, \ldots). Nonetheless, they have a high computational cost both in terms of time and memory. This makes their application difficult even for small and medium sample sizes ($n< 10^4$). This computational issue is addressed by first describing a new efficient and exact algorithm for kernel multiple change-point detection with an improved worst-case complexity that is quadratic in time and linear in space. It allows dealing with medium size signals (up to $n \approx 10^5$). Second, a faster but approximation algorithm is described. It is based on a low-rank approximation to the Gram matrix. It is linear in time and space. This approximation algorithm can be applied to large-scale signals ($n \geq 10^6$). These exact and approximation algorithms have been implemented in \texttt{R} and \texttt{C} for various kernels. The computational and statistical performances of these new algorithms have been assessed through empirical experiments. The runtime of the new algorithms is observed to be faster than that of other considered procedures. Finally, simulations confirmed the higher statistical accuracy of kernel-based approaches to detect changes that are not only in the mean. These simulations also illustrate the flexibility of kernel-based approaches to analyze complex biological profiles made of DNA copy number and allele B frequencies. An R package implementing the approach will be made available on github.

==> macros.tex <==
% \setlength{\topmargin}{-15mm}
% \setlength{\oddsidemargin}{-2mm}
% \setlength{\textwidth}{165mm}
% \setlength{\textheight}{250mm}

\numberwithin{equation}{section}
% \theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{lem}{Lemma}[section]
\newtheorem{prop}{Proposition}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{algo}{Procedure}[section]
\newtheorem{rk}{Remark}[section]
\newcommand{\prob}[1]{\mathbb{P}\left(#1 \right)}
\newcommand{\probi}[2]{\mathbb{P}_{#1}\left( #2 \right)}
\newcommand{\probc}[2]{\mathbb{P}\left(#1 \ | \ #2 \right)}
\newcommand{\probci}[3]{\mathbb{P}_{#1}\left(#2 \ | \ #3 \right)}

\newcommand{\esp}[1]{\mathbb{E}\left[#1 \right]}
\newcommand{\espi}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\Ln}{\widehat{L}_n}
\newcommand{\Lp}{\widehat{L}_p}
\newcommand{\sumIinEb}{\sum_{i\in\bar{e}}}
\newcommand{\som}[2]{\sum_{#1}^{#2}}
%\newcommand{\ind}[1]{I_{\{#1 \}}}
\newcommand{\f}[1]{ \widehat{f}_k( #1 ) }
\newcommand{\fe}[1]{ \widehat{f}_k(e, #1 ) }
\newcommand{\fep}[1]{ \widehat{f}_k(e', #1 ) }
\newcommand{\lpok}{\widehat{R}_p(k)}
\newcommand{\ldpok}{\widehat{R}^2_p(k)}
\newcommand{\cb}[2]{(_{#2}^{#1})}
\newcommand{\gp}[1]{\left(#1\right)}
\newcommand{\ga}[1]{\left\{#1\right\}}
\newcommand{\gc}[1]{\left[#1\right]}
\newcommand{\tito}[1]{o\left(#1\right)}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\Card}[1]{\mathrm{Card}\paren{ #1 }}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\1}{\mathds{1}}% indicatrice
\newcommand{\ind}[1]{\1_{\ga{#1}}}% indicatrice
\newcommand{\fn}[2]{\widehat{f}_k\left(#1;#2\right)}
%
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\croch}[1]{\left[\, #1 \,\right]}
\newcommand{\acc}[1]{\left\{ #1 \right\}}
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^2}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\normn}[1]{\left\| #1 \right\|_n}
\newcommand{\norminf}[1]{\left\| #1 \right\|_{\infty}}
\newcommand{\scal}[1]{\left< #1 \right>_2}
\newcommand{\scaln}[1]{\left< #1 \right>_n}
\newcommand{\st}{\, | \,}
\newcommand{\tq}{\mathrm{~s.t.~}} % tel que dans une définition d'ensemble
\newcommand{\guill}[1]{``#1''}% guillemets
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert} %joli abs
\newcommand{\mini}[2]{#1 \wedge #2}
\newcommand{\maxi}[2]{#1 \vee #2}
\renewcommand{\H}[1]{ \mathcal{H}\left( #1 \right)}
\def\lbr{\hbox{ $\mathrm{[}$\hskip -4.2pt {$\mathrm{[}\,$}}}
\def\rbr{\hbox{$\,\mathrm{]}$\hskip -4.2pt {$\mathrm{]}\,$}}}
\newcommand{\br}[1]{\left\lbr #1 \right\rbr}
\newcommand{\defegal}{:=} % egalite definissant la quantité de gauche
\newcommand{\egaldef}{=:} % egalite definissant la quantité de droite
\newcommand{\iid}{\textit{i.i.d.}\ }
\newcommand{\argmin}{\mathrm{Argmin}}
\newcommand{\Ref}{({\bf REFERENCES}) }
\newcommand{\ie}{{\it i.e.}\ }
\newcommand{\eg}{{\it e.g.}\ }

%
\newcommand{\F}{\mathcal{F}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\U}{\mathbb{U}}

\DeclareMathOperator{\pen}{pen}%penalite
\DeclareMathOperator{\crit}{crit}%critere
\DeclareMathOperator{\card}{Card} %cardinal
\DeclareMathOperator{\sign}{sign}%signe


\newcommand{\et}{{\it et al.}\ }
\newcommand{\ap}{{\it a priori}\ }
\newcommand{\Rk}{\textsc{Remark:}\ }
\newcommand{\Rks}{\textsc{Remarks:}\ }
\newcommand{\Open}{\textsc{Open question:}\ }
\newcommand{\homo}{homoscedastic\ }
\newcommand{\hetero}{heteroscedastic\ }
%
%
\newcommand{\ph}{\widehat{p}}
\newcommand{\sh}{\,\widehat{s}\,}
\newcommand{\mh}{\widehat{m}}
\newcommand{\sm}{s_m}
\newcommand{\shm}{\widehat{s}_m}
%\newcommand{\VF}{V-fold\ }
\newcommand{\Sm}{S_{m}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\Mn}{\mathcal{M}_n}
\renewcommand{\l}{\ell}
\newcommand{\Ss}{\mathcal{S}^*}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\X}{\mathcal{X}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\gn}{\gamma_n}
\newcommand{\CV}{cross-validation}
\newcommand{\Pg}{P\gamma}
\newcommand{\Pn}{P_n}
\newcommand{\PnW}{P_n^W}
\newcommand{\PnWc}{P_n^{\overline{W}}}
\newcommand{\Png}{P_n\gamma}
\newcommand{\g}{\gamma}
\newcommand{\perte}[1]{\ell\paren{s,#1\,}}
\newcommand{\risk}[1]{\E\croch{\ell\paren{s,#1\,}}}
\newcommand{\penh}{\widehat{\pen}}
\newcommand{\idpen}{\pen_{id}}
\newcommand{\Rh}{\widehat{R}}
\newcommand{\phil}{\varphi_{\lambda}}
\newcommand{\phill}{\varphi_{\lambda'}}
\newcommand{\bl}{\beta_{\lambda}}
\newcommand{\bll}{\beta_{\lambda'}}
\newcommand{\bhl}{\widehat{\beta}_{\lambda}}
\newcommand{\bhll}{\widehat{\beta}_{\lambda'}}
\newcommand{\al}{\alpha_{\lambda}}
\newcommand{\Al}{A_{\lambda}}
\newcommand{\Bl}{B_{\lambda}}
\newcommand{\All}{A_{\lambda'}}
\newcommand{\Bll}{B_{\lambda'}}
\newcommand{\all}{\alpha_{\lambda'}}
\newcommand{\ahl}{\widehat{\alpha}_{\lambda}}
\newcommand{\ahll}{\widehat{\alpha}_{\lambda'}}
\newcommand{\Il}{I_{\lambda}}
\newcommand{\Ill}{I_{\lambda'}}
\newcommand{\Bel}{\beta_{\lambda}}
\newcommand{\Ep}{\mathcal{E}_p}
\newcommand{\Sl}{S_{\lambda}}
\newcommand{\Sll}{S_{\lambda,\lambda'}}
\newcommand{\nl}{n_{\lambda}}
\newcommand{\silr}{\paren{\sigma_{\lambda}^r}^2}
\newcommand{\silb}{\paren{\sigma_{\lambda}^b}^2}
\newcommand{\Hbf}{{\bf H}}
\newcommand{\pih}{\widehat{\pi}}
\newcommand{\Lh}{\widehat{L}}
\newcommand{\Gh}{\widehat{G}}
\newcommand{\oh}{\widehat{\omega}}
\newcommand{\ol}{\omega_{\lambda}}
\newcommand{\MSEh}{\widehat{MSE}}
\newcommand{\Abf}{{\bf A}}
\newcommand{\Reg}{$\paren{Reg}$\ }
\newcommand{\Ad}{$\paren{Ad}$\ }
\newcommand{\Bor}{$\paren{Bor}$\ }
\newcommand{\Pol}{$\paren{Pol}$\ }
\newcommand{\Ran}{$\paren{Ran}$\ }
\newcommand{\Car}{$\paren{Car}$\ }
\newcommand{\Rac}{$\paren{Rac}$\ }
\newcommand{\Em}{E_m}
\newcommand{\Emh}{E_{\mh}}
\newcommand{\la}{\lambda}
\newcommand{\n}{\nu_n}
\newcommand{\Rhp}{\Rh_p}
\newcommand{\Rhpm}{\Rhp(m)}
\newcommand{\ERM}{\widehat{s}}
\newcommand{\ERMalg}{\ensuremath{\mbox{ERM}}}
%\newcommand{\lamm}{\lambda \in \Lambda_m}
\newcommand{\D}{\mathcal{D}}
\newcommand{\LPO}{\mathrm{LPO}}
\newcommand{\LOO}{\mathrm{LOO}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\penRad}{\mathrm{penRad}}
\newcommand{\Emp}{\mathrm{Emp}}
\newcommand{\BM}{\mathrm{BM}}
\newcommand{\penVF}{\mathrm{penVF}}
\newcommand{\VF}{\mathrm{VF}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\Dh}{\widehat{D}}
\newcommand{\pl}{p_{\lambda}}
\newcommand{\phl}{\widehat{p}_{\lambda}}
\newcommand{\Nb}{\mathrm{Nb}}





%%% Raccourcis Alain
\newcommand{\eb}{\bar e}
\newcommand{\es}{{\bar e}^{\sigma}}
\renewcommand{\et}{{\bar e}^{\tau}}
\newcommand{\Ab}{A^{\eb}}
\newcommand{\As}{A^{\es}}
\newcommand{\At}{A^{\et}}
\newcommand{\Enp}{\mathcal{E}_{n-p}}



==> runtimes.tex <==




For our heuristic we considered to parametrization either constant value of $p$ or $p=\sqrt{n}$. In the second case the worst
case complexity is quadratic as our exact algorithm, however the overhead is much smaller as can be seen in figure \ref{fig:timeandmemory} (Right).  Figure \ref{fig:timeandmemory} illustrates the fact that our exact algorithm is able to cope with signal of size $10^5$ in a matter of minutes whereas our heuristic is much faster and does it in a matter of a few seconds.

\begin{figure}
\begin{center}
\begin{tabular}{ccc}
KernSeg and quartic KCP & KernSeg and ECP & KernSeg Exact and Heuristic\\
\includegraphics[scale=0.3]{fig/RunTimeQuartic.png} &
\includegraphics[scale=0.3]{fig/RunTimeEcp_ALL_.png} &
\includegraphics[scale=0.3]{fig/RunTimeExactAndApprox.png}
\end{tabular}
\end{center}
\caption{(Left) Runtime for $n < 250$ of our dynamic programming algorithm as a function of the length of the signal (1-red) and a quartic computation of the cost matrix (2-violet).
(Middle) Runtime for $n < 2500$ of our dynamic programming algorithm as a function of the length of the signal (1-red) of ECP without permutation (2-blue) and ECP with the default number of permuations (3-green). (Right) Runtime for $n < 100000$ of our exact dynamic programming algorithm as a function of the length of the signal (1-red), of our heuristic with $p=\sqrt{n}$ (2-orange) and $p=100$ (3-black).}\label{fig:timeandmemory}. 
\end{figure}
 

